Multilevel Combinatorial Optimization Across Quantum Architectures

Emerging quantum processors provide an opportunity to explore new approaches for solving traditional problems in the post Moore's law supercomputing era. However, the limited number of qubits makes it infeasible to tackle massive real-world datasets directly in the near future, leading to new challenges in utilizing these quantum processors for practical purposes. Hybrid quantum-classical algorithms that leverage both quantum and classical types of devices are considered as one of the main strategies to apply quantum computing to large-scale problems. In this paper, we advocate the use of multilevel frameworks for combinatorial optimization as a promising general paradigm for designing hybrid quantum-classical algorithms. In order to demonstrate this approach, we apply this method to two well-known combinatorial optimization problems, namely, the Graph Partitioning Problem, and the Community Detection Problem. We develop hybrid multilevel solvers with quantum local search on D-Wave's quantum annealer and IBM's gate-model based quantum processor. We carry out experiments on graphs that are orders of magnitudes larger than the current quantum hardware size, and we observe results comparable to state-of-the-art solvers in terms of quality of the solution.

==> old.tex <==
\section{Results}\label{sec:results}
%added from local directory
% check
The classical part of ML-QLS is implemented in Python 3.7 using NetworkX~\cite{hagberg2008-rs} 
for network operations. The subproblem solvers are implemented using QA (D-Wave SAPI) and QAOA (IBM QisKit~\cite{Qiskit}). We also implemented a subproblem solver using the classical Gurobi solver~\cite{optimization2014inc-rs} for performance comparison (denoted ``Optimal'' in plots, as we allow it to solve each subproblem to optimality). %QA is run on \added[id=rs]{@Hayato add device info / citation}.
QAOA is run both on the high-performance IBM Qiskit Aer simulator~\cite{Qiskit}, as well as on the Poughkeepsie 20 qubit quantum computer available on the Oak Ridge National Laboratory (ORNL) IBM Q hub network. Our framework is modular and easily extendable. The novel subproblem solvers can be easily added as they become available. We used GNU Parallel for large-scale numerical experiments~\cite{tange_ole_2018_1146014}. The code is available on GitHub~\cite{code}.

The QAOA is implemented using the  SBPLX~\cite{rowan1991functional} optimizer to find the optimal variational parameters. We allow 2000 iterations for SBPLX to find optimal parameters for QAOA run on the simulator and 250 iterations for QAOA on the device. Due to the limitations of NISQ devices available in IBM Q hub network~\cite{Shaydulin2019}, we used the  RYRZ variational form~\cite{ibmqryrz-rs} (also known as a hardware-efficient ansatz) as the ansatz for our QAOA implementation. For the experiments run on IBM quantum device Poughkeepsie, we perform the variational parameter optimization on the simulator locally and run QAOA on the device via the IBM Q Experience cloud API. This is done due to the job queue limitations provided via the IBM Q Experience and we expect to be able to run QAOA variational parameter optimization fully on a device as more devices are becoming available on the cloud.



%%
In this work, we used the D-Wave 2000Q located at Los Alamos National Laboratory (LANL), which is the state-of-the-art quantum annealer at this time. It has up to 2048 qubits which are laid out in a special graph structure known as a Chimera graph. The Chimera graph is sparse, thus the device has sparse connectivity. Fully connected graphs as dense problems need to be embedded onto the device, which leads to the maximum size of 64 variables. In this work, we use the embedding algorithm described in ~\cite{boothby2016fast} %\added[id=is]{is there a name of the alg?} 
to calculate a complete embedding of the 64 variable problem. We found this embedding only once and reused it during our experiments. We utilize D-Wave's Solver API (SAPI) which is implemented in Python 2.7, to interact with the system. The D-Wave system is intrinsically a stochastic system, where solutions are sampled from a distribution corresponding to the lowest energy state. For each subproblem, the best solution out of 10,000 samples is returned. 


\begin{table*}[t]
\begin{center}
\begin{tabular}{ |c|c|c|c|c|c|c|c| } 
\hline 
 Network name & $|V|$ & $|E|$ & $d_{\mbox{avg}}$ & $d_{\mbox{max}}$  \\
 \hline
\texttt{SSS12} &	 21996 	& 1221028 &	 111.02 &	 722 \\
\texttt{4elt} &	 15606 &	 45878 &	 5.88 &	 10 \\
\texttt{bcsstk30} &	 28924 &	 1007284 &	 69.65 &	 218 \\
\texttt{cti} &	 16840 	& 48232 &	 5.73 & 	 6 \\
\texttt{data} &	 2851 &	 15093 	& 10.59 &	 17 \\
\texttt{roadNet-PA-20k} &	 20000 &	 26935 	& 2.69 &	 7 \\
\texttt{opsahl-powergrid} &	 4941 &	 6594 &	 2.67 &	 19 \\
\texttt{msc23052} &	 5722 &	 103391 &	 36.14 &	 125 \\
\texttt{finan512-10k} &	 10000 	& 28098 &	 5.62 &	 54 \\
 \hline
\end{tabular}
\caption{Properties of the networks used to evaluate ML-QLS. $d_{\mbox{avg}}$ is average degree, $d_{\mbox{max}}$ is maximum degree}
\label{tab:graph_prop}
\end{center}
\end{table*}

% exponent for the degree distribution == \gamma
% exponent for the community size distribution == \beta
% mixing parameter == \mu

\begin{table*}[t]
\begin{center}
\begin{tabular}{ |c|c|c|c|c|c|c|c| } 
\hline 
 Network name & $|V|$ & $|E|$ & $d_{\mbox{avg}}$ & $d_{\mbox{max}}$ & $\gamma$ & $\beta$ & $\mu$ \\
 \hline
 \texttt{GirvanNewman} & 10,000 & 75,000 & 15.0 & 15 & 1 & 1 & 0.1 \\ 
 \texttt{lancichinetti1} & 10,000 & 76,133 & 15.22 & 50 & 2 & 1 & 0.1 \\ 
 \hline
\end{tabular}
\caption{Properties of synthetic networks used in the Modularity evaluation. $d_{\mbox{avg}}$ is average degree, $d_{\mbox{max}}$ is maximum degree, $\gamma$ is the  exponent for the degree distribution, $\beta$ is the exponent for the community size distribution and $\mu$ is the mixing parameter. For a detailed discussion of the parameters the reader is referred to Ref.~\cite{Lancichinetti2008}}
\label{tab:mod_synth}
\end{center}
\end{table*}

%%
For the Graph Partitioning Problem, we evaluate ML-QLS on five graphs, four of which are drawn from The Graph Partitioning Archive~\cite{Soper2004} (\texttt{4elt}, \texttt{bcsstk30}, \texttt{cti} and \texttt{data}) and one from the set of hard to partition graphs
(\texttt{vsp\_msc10848\_300sep\_100in\_1Kout}, denoted in figures as \texttt{SSS12})~\cite{amg-sss12}. 
We compare the quality of the partitioning produced by ML-QLS with a classical state-of-the-art solver KaHIP~\cite{sandersschulz2013} and with the best known results from The Graph Partitioning Archive~\cite{Soper2004}. To evaluate the quality of the solution obtained by ML-QLS, we compare it to the state-of-the-art GP solver package KaHIP~\cite{sandersschulz2013}. Following the user guide~\cite{kahipguide}, we use the \texttt{kaffpaE} solver included in KaHIP together with the option {\tt --mh\_enable\_kabapE} for the high quality of partitioning for perfectly balanced parts. We use the option {\tt --preconfiguration=fast} to ensure results are compared with a single V-cycle. For the graphs from The Graph Partitioning Archive~\cite{Soper2004}, we normalize results by the smallest known cut as reported in the Archive, otherwise the results are normalized by the smallest cut found by any solver.

\begin{table}
\begin{center}
\begin{tabular}{ |c|c| } 
\hline 
 Network name & Best modularity\\
 \hline
 \texttt{finan512-10k}  & 0.499 \\
\texttt{GirvanNewman} & 0.459 \\
\texttt{lancichinetti1} & 0.452 \\
\texttt{msc23052}  & 0.499 \\
\texttt{opsahl-powergrid} & 0.497 \\
\texttt{roadNet-PA-20k} & 0.499 \\
 \hline
\end{tabular}
\caption{Highest modularity value found by all methods for a given problem. The highest possible modularity value for at most 2 communities is 0.5.}
\label{tab:mod_best}
\end{center}
\end{table}


\begin{figure*}[tb]
    \centering
    \subfloat[Mean]{\includegraphics[width=0.5\textwidth]{fig/hwsize_scaling_mean.pdf}}
    \hfill
    \subfloat[Standard deviation]{\includegraphics[width=0.5\textwidth]{fig/hwsize_scaling_std.pdf}}
    \caption{Modularity (Approximation ratio) as the function of the size of the subproblem (hardware size). The performance is projected using Gurobi as the subproblem solver and allowing it to solve each subproblem to optimality. The top plot presents the mean approximation ratio averaged over the entire benchmark. The bottom plot presents the standard deviation. As the hardware size increases, the quality of the solution found by ML-QLS improves.}
    \label{fig:hwsize_scaling}
\end{figure*}



\begin{figure}
    \centering
    \vspace{-1.5cm}
    \includegraphics[width=\textwidth, trim=0cm 4cm 0cm 0cm]{fig/MOD_barchart.pdf}
    \includegraphics[width=\textwidth]{fig/GP_barchart.pdf}
    % \vspace{-0.5cm}
    \caption{Quality of the solution and the number of iterations for all problems and solvers. The height of the bars is the median over 10 seeds. Error bars (black) are 25th and 75th percentiles. For the objective function (Cut or Modularity) all results are normalized by the best solution found by any solver (for Graph Partitioning this includes the best known cuts from The Graph Partitioning Archive~\cite{Soper2004}). Number of iterations is the number of calls to the subproblem solver (ML-QLS only).}
    \label{fig:barchart}
    \vspace{-0.25cm}
\end{figure}


For the Modularity Maximization Problem, we evaluate ML-QLS on six graphs. The graphs 
\texttt{roadNet-PA-20k} and \texttt{opsahl-powergrid} are real-world networks from the KONECT dataset~\cite{kunegis2013konect_rs}. Graphs \texttt{msc23052} and \texttt{finan512-10k} are taken from the graph archive presented in Ref.~\cite{Safro2011}. The graphs \texttt{finan512-10k} and \texttt{roadNet-PA-20k} are reduced to 10,000 and 20,000 nodes respectively by performing a breadth-first search from the median degree node. Note that due to the high diameter of these networks and their structure (portfolio optimization problem and road network), this preserves their structural properties. Graph properties are presented in Table~\ref{tab:graph_prop}. \texttt{GirvanNewman} is a synthetic graph generated using the model introduced by Girvan and Newman (GN)~\cite{Girvan2002}. \texttt{lancichinetti1} is a synthetic graph generated using a generalization of the GN model that allows for heterogeneity in the distributions of node degree and community size, introduced by Lancichinetti et al.~\cite{Lancichinetti2008}. Table~\ref{tab:mod_synth} shows the parameters used to generate the synthetic graphs. 


We compare the solution of ML-QLS with two classical clustering methods, Asynchronous Fluid Communities~\cite{pares2017fluid} (implemented in NetworkX~\cite{hagberg2008-rs}) and Spectral Clustering~\cite{shi2000normalized, von2007tutorial-rs} (implemented in Scikit-learn~\cite{scikit-learn}). Note that even though these methods solve the same problem (namely, Community Detection or clustering), they do not explicitly maximize modularity. Therefore, it is unfair to directly compare the modularity of the solution produced by them to ML-QLS, which is explicitly maximizing modularity. However, they provide a useful baseline. Moreover, since the maximum possible modularity for at most 2 communities is 0.5, the best solutions found by all methods are no more than 1\%--10\% away from the optimal (see Table~\ref{tab:mod_best})


The results are presented in Figure~\ref{fig:barchart}. We made all results available on Github~\cite{rawdata}. For each problem and method (except for QAOA on IBM Q Poughkeepsie quantum computer, labeled ``QAOA (IBMQ Poughkeepsie)'' in Figure~\ref{fig:barchart}), we perform ten runs of a single V-cycle with different seeds.  For ``QAOA (IBMQ Poughkeepsie)'', we perform just one run per each problem due to the limited access to quantum hardware. We observe that ML-QLS is capable of achieving results close to the optimal for all problems compared to other solvers. For Graph Partitioning (GP), Figure~\ref{fig:barchart} shows significant variability in the quality of the solution across different solvers and problem instances. This effect is also observed for the state-of-the-art GP solver KaHIP. This is partially due to the fact that we normalize the objectives to make them directly comparable. For example, for the graph 4elt the cut value presented in The Graph Partitioning Archive~\cite{Soper2004} is 139. Therefore, an \emph{absolute} difference of 28 edges in cut obtained by a solver translates into 20\% \emph{relative} difference presented in Figure~\ref{fig:barchart}. However, the same \emph{absolute} difference of 28 edges would translate into $\approx 0.44\%$ for the graph bcsstk30 (best known cut 6394). The graph \texttt{SSS12} is specifically designed to be hard for traditional Graph Partitioning frameworks~\cite{amg-sss12}. This explains the high variation in the performance of KaHIP on it.

It is worth noting that QAOA on the IBM quantum computers (see ``QAOA (IBM Q Poughkeepsie)'' in Figure~\ref{fig:barchart}) takes more iterations to converge to a solution compared to D-Wave. This is partially due to the fact that we perform the QAOA variational parameter optimization on the simulator and only run once with the optimized parameters on the device. As a result, the learned variational parameters do not include the noise profile of the device, limiting the quality of subproblem solutions. As devices become more easily available, we expect to be able to run full variational parameter optimization on the quantum hardware.

To project the performance improvements for future hardware, we simulate the performance of ML-QLS as a function of hardware (subproblem) size shown in Figure~\ref{fig:hwsize_scaling}. As the subproblem size increases, the average quality of the solution found by ML-QLS improves and variation in results decreases. This shows that performance of ML-QLS can be improved as larger size quantum devices and better quantum optimization routines are developed.


% ./results_as_a_function_of_hwsize_plot.py {/zfs/safrolab/share/graph_partitioning_results/pyomo/ML_QLS_pyomo_hw_sweep_0708_modularity*,/zfs/safrolab/share/graph_partitioning_results/dwave/*_modularity_*}

% \uselengthunit{in}\printlength{\columnwidth}
% \showthe\font


% for GP: 
% ./explore_partition_results.py {kaffpa_e.p,/zfs/safrolab/share/graph_partitioning_results/qaoa/ML_QLS_sim_2000_iter_0521_GP*,/zfs/safrolab/share/graph_partitioning_results/pyomo/ML_QLS_pyomo_hw64_0708_GP*,/zfs/safrolab/share/graph_partitioning_results/qaoa/ML_QLS_dev_2000_iter_0529_GP*,/zfs/safrolab/share/graph_partitioning_results/dwave/2019070[56]*_GP_*_hwsize_20*,/zfs/safrolab/share/graph_partitioning_results/dwave/rerun_find_embedding_fast_GP_vsp_msc10848_300sep_100in_1Kout_seed_*_hwsize_64*,/zfs/safrolab/share/graph_partitioning_results/dwave/find_embedding_fast_GP*_hwsize_64*} --plot


